Note on integrability of certain homogeneous Hamiltonian systems

In this paper we investigate a class of natural Hamiltonian systems with two degrees of freedom. The kinetic energy depends on coordinates but the system is homogeneous. Thanks to this property it admits, in a general case, a particular solution. Using this solution we derive necessary conditions for the integrability of such systems investigating differential Galois group of variational equations.

==> mathdef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                                %%%%
%%%%      this is my mathematical macros....        %%%%
%%%%                                                %%%%
%%%%  last update: 13.09.2004                      %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%          shortcuts for letters in different fonts in math mode
%%%%%
%%%%    bold
%%
%
\newcommand\ba{{\mathbf a}}
\newcommand\bb{{\mathbf b}}
\newcommand\bc{{\mathbf c}}
\newcommand\bd{{\mathbf d}}
\newcommand\be{{\mathbf e}}
\newcommand\bff{{\mathbf f}}
\newcommand\bg{{\mathbf g}}
\newcommand\bh{{\mathbf h}}
%\newcommand\bi{{\mathbf i}}
\newcommand\bj{{\mathbf j}}
\newcommand\bk{{\mathbf k}}
\newcommand\bl{{\mathbf l}}
%\newcommand\bm{{\mathbf m}}
\newcommand\bn{{\mathbf n}}
\newcommand\bo{{\mathbf o}}
\newcommand\bp{{\mathbf p}}
\newcommand\bq{{\mathbf q}}
\newcommand\br{{\mathbf r}}
%\newcommand\bs{{\mathbf s}}
\newcommand\bt{{\mathbf t}}
\newcommand\bx{{\mathbf x}}
\newcommand\bu{{\mathbf u}}
\newcommand\bv{{\mathbf v}}
\newcommand\bw{{\mathbf w}}
\newcommand\by{{\mathbf y}}
\newcommand\bz{{\mathbf z}}
\newcommand\bzero{{\mathbf 0}}

%
\newcommand\bA{{\mathbf A}}
\newcommand\bB{{\mathbf B}}
\newcommand\bC{{\mathbf C}}
\newcommand\bD{{\mathbf D}}
\newcommand\bE{{\mathbf E}}
\newcommand\bF{{\mathbf F}}
\newcommand\bG{{\mathbf G}}
\newcommand\bH{{\mathbf H}}
\newcommand\bI{{\mathbf I}}
\newcommand\bJ{{\mathbf J}}
\newcommand\bK{{\mathbf K}}
\newcommand\bL{{\mathbf L}}
\newcommand\bM{{\mathbf M}}
\newcommand\bN{{\mathbf N}}
\newcommand\bO{{\mathbf O}}
\newcommand\bP{{\mathbf P}}
\newcommand\bQ{{\mathbf Q}}
\newcommand\bR{{\mathbf R}}
\newcommand\bS{{\mathbf S}}
\newcommand\bT{{\mathbf T}}
\newcommand\bU{{\mathbf U}}
\newcommand\bV{{\mathbf V}}
\newcommand\bW{{\mathbf W}}
\newcommand\bX{{\mathbf X}}
\newcommand\bY{{\mathbf Y}}
\newcommand\bZ{{\mathbf Z}}
%
%%%%   snas serif
%%%
%%
%
%\newcommand\sfa{{\mathsf a}}
%\newcommand\sfb{{\mathsf b}}
%\newcommand\sfc{{\mathsf c}}
%\newcommand\sfd{{\mathsf d}}
%\newcommand\sfe{{\mathsf e}}
%\newcommand\sff{{\mathsf f}}
%\newcommand\sfg{{\mathsf g}}
%\newcommand\sfh{{\mathsf h}}
%\newcommand\sfi{{\mathsf i}}
%\newcommand\sfj{{\mathsf j}}
%\newcommand\sfk{{\mathsf k}}
%\newcommand\sfl{{\mathsf l}}
%\newcommand\sfm{{\mathsf m}}
%\newcommand\sfn{{\mathsf n}}
%\newcommand\sfo{{\mathsf o}}
%\newcommand\sfp{{\mathsf p}}
%\newcommand\sfq{{\mathsf q}}
%\newcommand\sfr{{\mathsf r}}
%\newcommand\sfs{{\mathsf s}}
%\newcommand\sft{{\mathsf t}}
%\newcommand\sfx{{\mathsf x}}
%\newcommand\sfu{{\mathsf u}}
%\newcommand\sfv{{\mathsf v}}
%\newcommand\sfw{{\mathsf w}}
%\newcommand\sfy{{\mathsf y}}
%\newcommand\sfz{{\mathsf z}}

%
\newcommand\sfA{{\mathsf A}}
\newcommand\sfB{{\mathsf B}}
\newcommand\sfC{{\mathsf C}}
\newcommand\sfD{{\mathsf D}}
\newcommand\sfE{{\mathsf E}}
\newcommand\sfF{{\mathsf F}}
\newcommand\sfG{{\mathsf G}}
\newcommand\sfH{{\mathsf H}}
\newcommand\sfI{{\mathsf I}}
\newcommand\sfJ{{\mathsf J}}
\newcommand\sfK{{\mathsf K}}
\newcommand\sfL{{\mathsf L}}
\newcommand\sfM{{\mathsf M}}
\newcommand\sfN{{\mathsf N}}
\newcommand\sfO{{\mathsf O}}
\newcommand\sfP{{\mathsf P}}
\newcommand\sfQ{{\mathsf Q}}
\newcommand\sfR{{\mathsf R}}
\newcommand\sfS{{\mathsf S}}
\newcommand\sfT{{\mathsf T}}
\newcommand\sfU{{\mathsf U}}
\newcommand\sfV{{\mathsf V}}
\newcommand\sfW{{\mathsf W}}
\newcommand\sfX{{\mathsf X}}
\newcommand\sfY{{\mathsf Y}}
\newcommand\sfZ{{\mathsf Z}}
%
%
%%%%   Euler fraktur
%%%
%%
%
\newcommand\efa{{\mathfrak a}}
\newcommand\efb{{\mathfrak b}}
\newcommand\efc{{\mathfrak c}}
\newcommand\efd{{\mathfrak d}}
\newcommand\efe{{\mathfrak e}}
\newcommand\eff{{\mathfrak f}}
\newcommand\efg{{\mathfrak g}}
\newcommand\efh{{\mathfrak h}}
\newcommand\efi{{\mathfrak i}}
\newcommand\efj{{\mathfrak j}}
\newcommand\efk{{\mathfrak k}}
\newcommand\efl{{\mathfrak l}}
\newcommand\efm{{\mathfrak m}}
\newcommand\efn{{\mathfrak n}}
\newcommand\efo{{\mathfrak o}}
\newcommand\efp{{\mathfrak p}}
\newcommand\efq{{\mathfrak q}}
\newcommand\efr{{\mathfrak r}}
\newcommand\efs{{\mathfrak s}}
\newcommand\eft{{\mathfrak t}}
\newcommand\efx{{\mathfrak x}}
\newcommand\efu{{\mathfrak u}}
\newcommand\efv{{\mathfrak v}}
\newcommand\efw{{\mathfrak w}}
\newcommand\efy{{\mathfrak y}}
\newcommand\efz{{\mathfrak z}}

%
\newcommand\efA{{\mathfrak A}}
\newcommand\efB{{\mathfrak B}}
\newcommand\efC{{\mathfrak C}}
\newcommand\efD{{\mathfrak D}}
\newcommand\efE{{\mathfrak E}}
\newcommand\efF{{\mathfrak F}}
\newcommand\efG{{\mathfrak G}}
\newcommand\efH{{\mathfrak H}}
\newcommand\efI{{\mathfrak I}}
\newcommand\efJ{{\mathfrak J}}
\newcommand\efK{{\mathfrak K}}
\newcommand\efL{{\mathfrak L}}
\newcommand\efM{{\mathfrak M}}
\newcommand\efN{{\mathfrak N}}
\newcommand\efO{{\mathfrak O}}
\newcommand\efP{{\mathfrak P}}
\newcommand\efQ{{\mathfrak Q}}
\newcommand\efR{{\mathfrak R}}
\newcommand\efS{{\mathfrak S}}
\newcommand\efT{{\mathfrak T}}
\newcommand\efU{{\mathfrak U}}
\newcommand\efV{{\mathfrak V}}
\newcommand\efW{{\mathfrak W}}
\newcommand\efX{{\mathfrak X}}
\newcommand\efY{{\mathfrak Y}}
\newcommand\efZ{{\mathfrak Z}}
%
%
%%%% caligraphic
%%%
%%
%
\newcommand\cA{{\mathcal A}}
\newcommand\cB{{\mathcal B}}
\newcommand\cC{{\mathcal C}}
\newcommand\cD{{\mathcal D}}
\newcommand\cE{{\mathcal E}}
\newcommand\cF{{\mathcal F}}
\newcommand\cG{{\mathcal G}}
\newcommand\cH{{\mathcal H}}
\newcommand\cI{{\mathcal I}}
\newcommand\cJ{{\mathcal J}}
\newcommand\cK{{\mathcal K}}
\newcommand\cL{{\mathcal L}}
\newcommand\cM{{\mathcal M}}
\newcommand\cN{{\mathcal N}}
\newcommand\cO{{\mathcal O}}
\newcommand\cP{{\mathcal P}}
\newcommand\cQ{{\mathcal Q}}
\newcommand\cR{{\mathcal R}}
\newcommand\cS{{\mathcal S}}
\newcommand\cT{{\mathcal T}}
\newcommand\cU{{\mathcal U}}
\newcommand\cV{{\mathcal V}}
\newcommand\cW{{\mathcal W}}
\newcommand\cX{{\mathcal X}}
\newcommand\cY{{\mathcal Y}}
\newcommand\cZ{{\mathcal Z}}
%
%%%% sript
%%%
%%
%
\newcommand\scA{{\mathscr A}}
\newcommand\scB{{\mathscr B}}
\newcommand\scC{{\mathscr C}}
\newcommand\scD{{\mathscr D}}
\newcommand\scE{{\mathscr E}}
\newcommand\scF{{\mathscr F}}
\newcommand\scG{{\mathscr G}}
\newcommand\scH{{\mathscr H}}
\newcommand\scI{{\mathscr I}}
\newcommand\scJ{{\mathscr J}}
\newcommand\scK{{\mathscr K}}
\newcommand\scL{{\mathscr L}}
\newcommand\scM{{\mathscr M}}
\newcommand\scN{{\mathscr N}}
\newcommand\scO{{\mathscr O}}
\newcommand\scP{{\mathscr P}}
\newcommand\scQ{{\mathscr Q}}
\newcommand\scR{{\mathscr R}}
\newcommand\scS{{\mathscr S}}
\newcommand\scT{{\mathscr T}}
\newcommand\scU{{\mathscr U}}
\newcommand\scV{{\mathscr V}}
\newcommand\scW{{\mathscr W}}
\newcommand\scX{{\mathscr X}}
\newcommand\scY{{\mathscr Y}}
\newcommand\scZ{{\mathscr Z}}
%

%%%
%%%%  definition of font for vectors - my choice is bold italic
%%%
\newcommand\mvector{\boldsymbol}

\newcommand\va{\mvector{a}}
\newcommand\vb{\mvector{b}}
\newcommand\vc{\mvector{c}}
\newcommand\vd{\mvector{d}}
\newcommand\ve{\mvector{e}}
\newcommand\vf{\mvector{f}}
\newcommand\vg{\mvector{g}}
\newcommand\vh{\mvector{h}}
\newcommand\vi{\mvector{i}}
\newcommand\vj{\mvector{j}}
\newcommand\vk{\mvector{k}}
\newcommand\vl{\mvector{l}}
\newcommand\vm{\mvector{m}}
\newcommand\vn{\mvector{n}}
\newcommand\vo{\mvector{o}}
\newcommand\vp{\mvector{p}}
\newcommand\vq{\mvector{q}}
\newcommand\vr{\mvector{r}}
\newcommand\vs{\mvector{s}}
\newcommand\vt{\mvector{t}}
\newcommand\vu{\mvector{u}}
\newcommand\vv{\mvector{v}}
\newcommand\vw{\mvector{w}}
\newcommand\vx{\mvector{x}}
\newcommand\vy{\mvector{y}}
\newcommand\vz{\mvector{z}}
\newcommand\vA{\mvector{A}}
\newcommand\vB{\mvector{B}}
\newcommand\vC{\mvector{C}}
\newcommand\vD{\mvector{D}}
\newcommand\vE{\mvector{E}}
\newcommand\vF{\mvector{F}}
\newcommand\vG{\mvector{G}}
\newcommand\vH{\mvector{H}}
\newcommand\vI{\mvector{I}}
\newcommand\vJ{\mvector{J}}
\newcommand\vK{\mvector{K}}
\newcommand\vL{\mvector{L}}
\newcommand\vM{\mvector{M}}
\newcommand\vN{\mvector{N}}
\newcommand\vO{\mvector{O}}
\newcommand\vP{\mvector{P}}
\newcommand\vQ{\mvector{Q}}
\newcommand\vR{\mvector{R}}
\newcommand\vS{\mvector{S}}
\newcommand\vT{\mvector{T}}
\newcommand\vU{\mvector{U}}
\newcommand\vV{\mvector{V}}
\newcommand\vW{\mvector{W}}
\newcommand\vX{\mvector{X}}
\newcommand\vY{\mvector{Y}}
\newcommand\vZ{\mvector{Z}}
%
\newcommand\valpha{\mvector{\alpha}}
\newcommand\vbeta{\mvector{\beta}}
\newcommand\vtheta{\mvector{\theta}}
\newcommand\vdelta{\mvector{\delta}}
\newcommand\veta{\mvector{\eta}}
\newcommand\vxi{\mvector{\xi}}
\newcommand\vchi{\mvector{\chi}}
\newcommand\vtau{\mvector{\tau}}
\newcommand\vrho{\mvector{\rho}}
\newcommand\vmu{\mvector{\mu}}
\newcommand\vlambda{\mvector{\lambda}}
\newcommand\vLambda{\mvector{\Lambda}}
\newcommand\vgamma{\mvector{\gamma}}
\newcommand\vGamma{\mvector{\Gamma}}
\newcommand\vvGamma{\mvector{\varGamma}}
\newcommand\vsigma{\mvector{\sigma}}
\newcommand\vomega{\mvector{\omega}}
\newcommand\vOmega{\mvector{\Omega}}
\newcommand\vsigm{\mvector{\sigma}}
\newcommand\vvarphi{\mvector{\varphi}}
\newcommand\vpsi{\mvector{\psi}}
\newcommand\vPhi{\mvector{\Phi}}
\newcommand\vXi{\mvector{\Xi}}
\newcommand\vzero{\mvector{0}}
\newcommand\vveps{\mvector{\varepsilon}}
%
%
%
%%% font for most common fields and rings
%%
%
\newcommand\field{\mathbb}
\newcommand\A{\field{A}}
\newcommand\R{\field{R}}
\newcommand\bbS{\mathbb{S}}
\newcommand\EE{\field{E}}
\newcommand\C{\field{C}}
\newcommand\Z{\field{Z}}
\newcommand\M{\field{M}}
\newcommand\N{\field{N}}
\newcommand\Q{\field{Q}}
\newcommand\K{\field{K}}
\newcommand\T{\field{T}}
\newcommand\bbH{\field{H}}
\newcommand\bbP{\mathbb{P}}
\newcommand\II{\field{I}}
\newcommand\PP{\mathbb{P}}
%
%
\newcommand\balpha{\boldsymbol{\alpha}}
\newcommand\bgamma{\boldsymbol{\gamma}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\bOmega{\boldsymbol{\Omega}}
\newcommand\bomega{\boldsymbol{\omega}}
\newcommand\bGamma{\boldsymbol{\Gamma}}
\newcommand\bTheta{\boldsymbol{\Theta}}
\newcommand\bLambda{\boldsymbol{\Lambda}}
\newcommand\bPi{\boldsymbol{\Pi}}
\newcommand\bmu{\boldsymbol{\mu}}
\newcommand\bphi{\boldsymbol{\varphi}}
\newcommand\bxi{\boldsymbol{\xi}}
\newcommand\bXi{\boldsymbol{\Xi}}
\newcommand\brho{\boldsymbol{\rho}}
\newcommand\bupsilon{\boldsymbol{\upsilon}}
\newcommand\vPi{\boldsymbol{\Pi}}
\newcommand\const{\operatorname{const}}
\newcommand\vect{\operatorname{Vect}}
\newcommand\vspan{\operatorname{span}}
\newcommand\supp{\operatorname{Supp}}
\newcommand\Div{\operatorname{div}}
\newcommand\rank{\operatorname{rank}}
\newcommand\diag{\operatorname{diag}}
\newcommand\sign{\operatorname{sign}}
%\newcommand\vspan{\operatorname{span}}
\renewcommand\Re{\operatorname{Re}}
\renewcommand\Im{\operatorname{Im}}
\newcommand\im{\operatorname{im}}
\newcommand\tr{\operatorname{Tr}}
\newcommand\res{\operatorname{res}}
\newcommand\result{\operatorname{Res}}
 \newcommand\mult{\operatorname{mult}}
 \newcommand\spectr{\operatorname{spectr}}
\newcommand\ord{\operatorname{ord}}
\newcommand\grad{\operatorname{grad}}
\newcommand\Sol{\operatorname{Sol}}
%\newcommand\arg{\operatorname{arg}}
\newcommand\lt{\operatorname{\mbox{\textsc{lt}}}}
\newcommand\card{\operatorname{card}}
\newcommand\trdeg{\operatorname{tr.\!deg}}
\newcommand\gdeg{\operatorname{\deg_{\vgamma}}}
\newcommand\sdeg{\operatorname{\mbox{$\vsigma$}-deg}}
\newcommand\ldeg{\operatorname{\mbox{$\vlambda$}-deg}}
\newcommand\id{\operatorname{\mathrm{Id}}}
\newcommand\sym{\operatorname{\small\mbox{$\circledS$}}}
%\newcommand\idn{\operatorname{\mathrm{Id}_{\mbox{n}}}}
%%%%
%%%    romman letters used in math mode
%%%
\newcommand\gal{\operatorname{Gal}}
\newcommand\rmd{\mathrm{d}}
\newcommand\SLtwoC{\ensuremath{\mathrm{SL}(2,\C)}}
\newcommand\CPOne{\ensuremath{\C\mathbb{P}^1}}
\newcommand\CP{\ensuremath{\C\bbP}}
\newcommand\VE[1]{\ensuremath{\mathrm{VE}_{#1}}}
\newcommand\EX[1]{\ensuremath{\mathrm{EX}_{#1}}}
\newcommand\PV[1]{\ensuremath{\mathrm{PV}{#1}}}
\newcommand\rmi{\mathrm{i}\mspace{1mu}}
\newcommand\rme{\mathrm{e}}
\DeclareMathOperator{\pv}{PV}
%
\newcommand\Dt{\frac{\mathrm{d}\phantom{t} }{\mathrm{d}\mspace{1mu}
t}}
\newcommand\Dx{\frac{\mathrm{d}\phantom{x} }{\mathrm{d}x}}
\newcommand\Dr{\frac{\mathrm{d}\phantom{r} }{\mathrm{d}r}}
\newcommand\Dp{\frac{\mathrm{d}\phantom{\phi} }{\mathrm{d}\phi}}
\newcommand\Dy{\frac{\mathrm{d}\phantom{y} }{\mathrm{d}y}}
\newcommand\Dz{\frac{\mathrm{d}\phantom{z} }{ \mathrm{d}z}}
\newcommand\Dwz{\frac{\rmd w }{\mathrm{d} z}}
\newcommand\Dtt{\frac{\mathrm{d}^2\phantom{t} }{\mathrm{d}t^2}}
\newcommand\oder[2]{\dfrac{\mathrm{d} #1 }{\mathrm{d} #2}}
\newcommand\pder[2]{\dfrac{\partial #1 }{\partial #2}}
\newcommand\Dtk[1]{\frac{\mathrm{d}^{#1}\phantom{t}
}{\mathrm{d}\mspace{1mu} t^{#1}}}
\newcommand\Dxx{\frac{\mathrm{d}^2\phantom{x} }{\mathrm{d}x^2}}
\newcommand\Dttt{\frac{\mathrm{d}^3\phantom{t} }{\mathrm{d}t^3}}
\newcommand\Dxxx{\frac{\mathrm{d}^3\phantom{x} }{\mathrm{d}x^3}}
 
%%%
%
%----> absolute value, norm and complex conjugate
%
\newcommand\abs[1]{\lvert #1 \rvert}
\newcommand\norm[1]{\lVert #1 \rVert}
\newcommand\cc[1]{\overline#1}
\newcommand\figref[1]{Fig.~\ref{#1}}
\newcommand\scalar[2]{\langle \mvector{#1},\mvector{#2}\rangle}
\newcommand\pairing[2]{\langle {#1}, {#2}\rangle}
%
%  rscalar does not change the apperance of its arguments
%
\newcommand\rscalar[2]{\langle #1, #2\rangle}
%
% elliptic functions of Jacobi
%
\newcommand\cn{\operatorname{cn}}
\newcommand\sn{\operatorname{sn}}
\newcommand\dn{\operatorname{dn}}
\newcommand\sk{\operatorname{S}_{\kappa}}
\newcommand\ck{\operatorname{C}_{\kappa}}
\newcommand\tk{\operatorname{T}_{\kappa}}
%
%
\newcommand\bfi[1]{{\bfseries\itshape{#1}}}
\newcommand\cpoly{\C[x_1,\ldots,x_n]}
\newcommand\crat{\C(x_1,\ldots,x_n)}
%
\newcommand\mtext[1]{\quad\text{#1}\quad}
\newcommand\mnote[1]{\marginpar{\tiny{#1}}}
\newcommand\defset[2]{\left\{{#1}\;\vert \;\; {#2} \,\right\}}
\newcommand\deftuple[2]{\left({#1}\;\vert \;\; {#2} \,\right)}

